Graphical Models: An Extension to Random Graphs, Trees, and Other Objects

In this work, we consider an extension of graphical models to random graphs, trees, and other objects. To do this, many fundamental concepts for multivariate random variables (e.g., marginal variables, Gibbs distribution, Markov properties) must be extended to other mathematical objects; it turns out that this extension is possible, as we will discuss, if we have a consistent, complete system of projections on a given object. Each projection defines a marginal random variable, allowing one to specify independence assumptions between them. Furthermore, these independencies can be specified in terms of a small subset of these marginal variables (which we call the atomic variables), allowing the compact representation of independencies by a directed graph. Projections also define factors, functions on the projected object space, and hence a projection family defines a set of possible factorizations for a distribution; these can be compactly represented by an undirected graph. The invariances used in graphical models are essential for learning distributions, not just on multivariate random variables, but also on other objects. When they are applied to random graphs and random trees, the result is a general class of models that is applicable to a broad range of problems, including those in which the graphs and trees have complicated edge structures. These models need not be conditioned on a fixed number of vertices, as is often the case in the literature for random graphs, and can be used for problems in which attributes are associated with vertices and edges. For graphs, applications include the modeling of molecules, neural networks, and relational real-world scenes; for trees, applications include the modeling of infectious diseases, cell fusion, the structure of language, and the structure of objects in visual scenes. Many classic models are particular instances of this framework.

==> frontmatter2.tex <==
%% Front matter for for FnT Machine Learning
%% (c) 2013 Neal Parikh (Stanford University)
%% 
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1 
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1 
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[0.3em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

\if@openright % -- for 'book' version
\parindent \z@

% title page
\thispagestyle{empty}
\vspace*{\fill}
\begin{flushright}
\begin{minipage}{0.8\textwidth}
\begin{flushright}
\renewcommand{\baselinestretch}{1.1}
\sffamily\bfseries\huge 
\@title
\end{flushright}
\end{minipage}
\end{flushright}
\vspace*{\fill}

% title+author page
\cleardoublepage
\thispagestyle{empty}

\begin{flushright}
{\renewcommand{\baselinestretch}{1.2}
\sffamily\Huge\bfseries \@title\par}
\vspace{3ex}
\noindent\rule{\textwidth}{2pt}
\vspace{1ex}\par

\begingroup
\def\and{%
  \end{tabular}%
  \par\vspace*{1.5ex}
  \begin{tabular}[t]{r@{}}
  \bfseries}

  \fontsize{13}{15}\selectfont\sffamily
\begin{tabular}[t]{r@{}}
    \bfseries
    \@author
\end{tabular}
\endgroup
\vfill
\includegraphics[width=53bp]{now_logo}\\
\includegraphics[width=81bp]{essence_logo}\\
Boston --- Delft
\end{flushright}

% publisher page
\newpage
\thispagestyle{empty}
\begingroup

\parskip6pt

{\bfseries\sffamily\Large \@journaltitleprefix\ \@journaltitle}
\footnotesize

\vfill

{\itshape Published, sold and distributed by:}\\
now Publishers Inc.\\
PO Box 1024\\
Hanover, MA\ 02339\\
United States\\
Tel.\ +1-781-985-4510\\
www.nowpublishers.com\\
sales@nowpublishers.com

{\itshape Outside North America:}\\
now Publishers Inc.\\
PO Box 179\\
2600 AD Delft\\
The Netherlands\\
Tel.\ +31-6-51115274

The preferred citation for this publication is

{\raggedright
\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
\@pubyear.\par}

{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
acid-free paper.}

ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner

\vfill

\fontsize{8}{9}\selectfont
All rights reserved. No part of this publication may be
reproduced, stored in a retrieval system, or transmitted in any form
or by any means, mechanical, photocopying, recording or otherwise,
without prior written permission of the publishers.

Photocopying. In the USA: This journal is registered at the Copyright
Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923. 
Authorization to photocopy items for
internal or personal use, or the internal or personal use of specific
clients, is granted by now Publishers Inc for users registered with 
the Copyright Clearance Center (CCC).
The `services' for users can be found on the internet at:
www.copyright.com

For those organizations that have been granted a photocopy license, a
separate system of payment has been arranged. Authorization does not
extend to other kinds of copying, such as that for general
distribution, for advertising or promotional purposes, for creating
new collective works, or for resale.  In the rest of the world:
Permission to photocopy must be obtained from the copyright
owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
sales@nowpublishers.com

now Publishers Inc. has an exclusive license to publish this
material worldwide. Permission to use this content must be obtained from
the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
sales@nowpublishers.com\par
\endgroup

% editorial board
\newpage
\thispagestyle{empty}
\begin{center}
\sffamily\LARGE
{\bfseries \@journaltitleprefix\ \@journaltitle}\\
{Volume \@volume, Issue \@issue, \@pubyear}\\
{\bfseries Editorial Board}
\end{center}

\vspace{12pt}

\ifnum\chiefeditorcount>1
{\sffamily\bfseries Editors-in-Chief}
{\footnotesize
\begin{multicols}{2}
\@chiefeditors
\end{multicols}}
\else
{\sffamily\bfseries Editor-in-Chief}\par
\vspace*{10pt}
\begin{footnotesize}
\begin{tabular}[t]{@{}l}
\@chiefeditors \\
\end{tabular}
\end{footnotesize}
\vspace*{10pt}
\fi

{\sffamily \bfseries Editors}
{\footnotesize %\fontsize{9}{11}\selectfont
\begin{multicols}{3}
\raggedcolumns
\@editors
\end{multicols}}%

% editorial scope
\newpage % page vi -- blank
\thispagestyle{empty}
\begin{center}
{\sffamily\bfseries\LARGE Editorial Scope}
\end{center}

\vspace{18pt}

{\bfseries\large\sffamily Topics}\\

\@journaltopicintro

\fontsize{10}{13}\selectfont
\begin{multicols}{2}
    \raggedright
    \@journaltopics
\end{multicols}

{\bfseries\large\sffamily Information for Librarians}\\

\@libraryinfo\par

\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
%{\hangindent=3.5ex
%\hangafter=1
%\@journaltitleprefix\ \@journaltitle\par}%
%Vol.~\@volume, No.~\@issue\ (\@pubyear) 
%\@firstpage--\@lastpage\\
%{\hangindent=3.5ex
%\hangafter=1
%\copyright\ \@copyrightyear\ \@copyrightowner\par}%
%DOI: \@doi}\hss
%\vbox{\hsize=.4\textwidth 
    \raggedleft
    %\includegraphics[width=53bp]{now_logo}\\
    %\includegraphics[width=81bp]{essence_logo}\\
    \par
}}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{now Publishers Inc.}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Machine Learning}

\journalchiefeditor{\textbf{Michael Jordan} \\
University of California, Berkeley \\
United States}

\journaleditor{Peter Bartlett \\ \emph{UC Berkeley}} 
\journaleditor{Yoshua Bengio \\ \emph{University of Montreal}} 
\journaleditor{Avrim Blum \\ \emph{CMU}} 
\journaleditor{Craig Boutilier \\ \emph{University of Toronto}} 
\journaleditor{Stephen Boyd \\ \emph{Stanford University}} 
\journaleditor{Carla Brodley \\ \emph{Tufts University}} 
\journaleditor{Inderjit Dhillon \\ \emph{UT Austin}} 
\journaleditor{Jerome Friedman \\ \emph{Stanford University}} 
\journaleditor{Kenji Fukumizu \\ \emph{ISM, Japan}} 
\journaleditor{Zoubin Ghahramani \\ \emph{University of Cambridge}} 
\journaleditor{David Heckerman \\ \emph{Microsoft Research}} 
\journaleditor{Tom Heskes \\ \emph{Radboud University} \columnbreak} 
\journaleditor{Geoffrey Hinton \\ \emph{University of Toronto}} 
\journaleditor{Aapo Hyvarinen \\ \emph{HIIT, Finland}} 
\journaleditor{Leslie Pack Kaelbling \\ \emph{MIT}} 
\journaleditor{Michael Kearns \\ \emph{UPenn}} 
\journaleditor{Daphne Koller \\ \emph{Stanford University}} 
\journaleditor{John Lafferty \\ \emph{University of Chicago}} 
\journaleditor{Michael Littman \\ \emph{Brown University}} 
\journaleditor{Gabor Lugosi \\ \emph{Pompeu Fabra University}} 
\journaleditor{David Madigan \\ \emph{Columbia University}} 
\journaleditor{Pascal Massart \\ \emph{University of Paris-Sud}} 
\journaleditor{Andrew McCallum \\ \emph{UMass Amherst}} 
\journaleditor{Marina Meila \\ \emph{University of Washington} \columnbreak} 
\journaleditor{Andrew Moore \\ \emph{CMU}} 
\journaleditor{John Platt \\ \emph{Microsoft Research}} 
\journaleditor{Luc de Raedt \\ \emph{University of Freiburg}} 
\journaleditor{Christian Robert \\ \emph{U Paris-Dauphine}} 
\journaleditor{Sunita Sarawagi \\ \emph{IIT Bombay}} 
\journaleditor{Robert Schapire \\ \emph{Princeton University}} 
\journaleditor{Bernhard Schoelkopf \\ \emph{MPI T\"{u}bingen}} 
\journaleditor{Richard Sutton \\ \emph{University of Alberta}} 
\journaleditor{Larry Wasserman \\ \emph{CMU}} 
\journaleditor{Bin Yu \\ \emph{UC Berkeley}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles on the theory, algorithms and applications of machine learning, including the following topics:}

\journaltopics{
\begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive, and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
}

\journallibraryinfo{%
  Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  Volume~\@volume, 6 issues. ISSN paper version 1935-8237.
  ISSN online version 1935-8245.
  Also available as a combined paper and online
  subscription.
}

\endinput

